FluidML: Fast and Memory Efficient Inference Optimization

Machine learning models deployed on edge devices have enabled numerous exciting new applications, such as humanoid robots, AR glasses, and autonomous vehicles. However, the computing resources available on these edge devices are not catching up with the ever-growing number of parameters in these models. As the models become bigger and more complicated, the novel yet sophisticated structure challenges the inference runtime optimization. We present FluidML, a generic runtime memory management and optimization framework that can flexibly transform the model execution blueprint to achieve faster and more memory-efficient inference. Evaluations across different platforms show that FluidML can consistently reduce the end-to-end inference latency by up to 25.38% for popular language models and reduce peak memory usage by up to 41.47%, compared to state-of-the-art approaches. FluidML is of ~30K line of codes, built for general-purpose usage, and will be released as an open-source inference runtime optimization framework to the community.

==> section/0_abstract_text.tex <==
ML-EXray: Visibility to ML Deployment on the Edge

Benefited from expanding cloud infrastructure, today's neural networks have increasingly high performance trained on the cloud.  Model researchers spent months of sweat competing for an extra few percent of model accuracy. However, when these models are actually deployed on edge devices in practice, very often, the performance is dropping over 10% all of a sudden without obvious reasons. The key challenge is that there is not much visibility to ML inference execution on edge devices, and very little awareness of potential issues during the edge deployment process. ML-EXray provides visibility to layer-level details of the ML execution, helps developers analyze and debug cloud-to-edge deployment issues. More often than not, the reason does not only lie in the model itself, but every operation throughout the data flow and the deployment process. Evaluations show that ML-EXray can effectively catch deployment issues, such as pre-processing bugs, quantization issues, suboptimal kernels; using ML-EXray, users need to write less than 15 line of code to fully examine the edge deployment pipeline; eradicating these issues, ML-EXray can correct model performance by up to 30%, pinpoint error-prune layers, guide users to optimize kernel execution latency by two orders of magnitude. Code and APIs will be released as a multi-lingual instrumentation library and a Python deployment validation library.

==> section/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> section/artifact.tex <==
\section{Artifact Appendix}


% \newcommand{\DOI}{https://doi.org/10.5281/zenodo.6042894}
\newcommand{\DOI}{https://doi.org/10.5281/zenodo.6338677}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

This artifact includes the ML-EXray library, the instrumentation APIs in C++, JAVA, and Python for TensorFlow Lite inference monitoring, as well as a full-fledged android application for image classification. The demo app and python examples can be used to reproduce most of the results. 

\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}
  \item {\bf Compilation: Android studio with bazel plugin}
  \item {\bf Binary: Android application binaries (apk)}
  \item {\bf Data set: subset of Imagenet and COCO, IMDB reviews, speech commands dataset.}
  \item {\bf Run-time environment: Ubuntu 20.04}
  \item {\bf Hardware: Android Devices (tested on Pixel4 and Pixel3}
  \item {\bf Metrics: Accuracy, per-layer mismatch in root mean square error, latency}
  \item {\bf Output: log files for each inference}
  \item {\bf How much disk space required (approximately)?: 100G}
  \item {\bf How much time is needed to prepare workflow (approximately)?: 1 day}
  \item {\bf How much time is needed to complete experiments (approximately)?: 1 week}
  \item {\bf Publicly available?: Yes}
  \item {\bf Code licenses (if publicly available)?: mit}
  \item {\bf Data licenses (if publicly available)?: mit}
  \item {\bf Archived (provide DOI)?:\\ \DOI}
\end{itemize}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How delivered}

\url{https://github.com/hangqiu/ML-EXray}

\noindent
\url{\DOI}

\subsubsection{Hardware dependencies}
Most of the results can be reproduced both on ubuntu 20.04 workstations as well as using an android device. However, edge devices such as android phones or EdgeTPUs can generate more diverse and interesting traces.



\subsubsection{Software dependencies}
ML-EXray is built with bazel. It is also very tightly integrated into the android demo application we developed, which also requires Android studio with bazel plugin, android sdk and ndk. Android studio comes in conveniently as an IDE and android emulator.

Other software dependencies include:
{\small
\begin{itemize}
\item \texttt{Android Studio Arctic Fox 2020.3.1}
\vspace{-2mm}
\item \texttt{Android Studio Bazel plugin}
\vspace{-2mm}
\item \texttt{Android SDK 11.0}
\vspace{-2mm}
\item \texttt{Android NDK 21.4.7075529}
\vspace{-2mm}
\item \texttt{JDK (default-jdk)}
\vspace{-2mm}
\item \texttt{Java Runtime Environment (JRE)}
\vspace{-2mm}
\item \texttt{Android SDK Build-tools 30.0.3}
\vspace{-2mm}
\item \texttt{Android Emulator 30.8.4 (need qemu\_kvm)}
\vspace{-2mm}
\item \texttt{opencv}
\vspace{-2mm}
\item \texttt{tensorflow\_datasets}
\vspace{-2mm}
\item \texttt{tensorflow\_hub}
\vspace{-2mm}
\item \texttt{tensorflow\_io}
\vspace{-2mm}
\item \texttt{pandas}
\vspace{-2mm}
\item \texttt{seaborn}
\vspace{-2mm}
\item \texttt{numpy}
\vspace{-2mm}
\item \texttt{sklearn}
\end{itemize}
}


\subsubsection{Data sets}

The artifact uses subsets of various popular benchmark datasets including Imagenet 2012, COCO2014, COCO2017, Speech Commands, IMDB reviews. The datasets and the links are included in the github repo. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

We provide the app binaries in the artifact as well as the source code to build the same binaries. To build the project, load and compile the project in android studio as a bazel project using bazel import. Download android SDK and NDK from the SDK manager of android studio. Specify SDK NDK path in WORKSPACE file.

\newcommand{\forceindent}{\leavevmode{\parindent=1em\indent}}

\textit{\small
android\_sdk\_repository(\\
\forceindent name = ``androidsdk",\\
\forceindent path = ``PathToAndroidRoot/Sdk",\\
)}

\textit{\small
android\_ndk\_repository(\\
\forceindent name = ``androidndk",\\
\forceindent path = ``PathToAndroidRoot/Sdk/ndk/21.4.7075529",\\
)
}

\noindent
Compile the bazel target:

$//examples/android/TFliteCppApp:edgemlinsight$ with arch flag e.g. $--config=android\_arm64$,
or equivalently use bazel commands as follows


{\small
% \begin{itemize}
% \item 
\vspace{2mm}
\noindent
\texttt{bazel build //examples/android/TFliteCppApp:
edgemlinsight --config=android\_arm64}
% \end{itemize}
}

Note: before using bazel, make sure to download all dependencies, including Android SDK, NDK using android studio, and specify the path in WORKSPACE file.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
Reproducing the traces of different edge ML executions requires running the app with different configurations (documented in README.md). The reference pipelines and traces that are not dependent on hardware can be run on ubuntu workstation using Python scripts under $edgeml/python/src/MLEXray/Model\_Runner/
$. 

Once the logs are generated, the Python scripts documented in scripts/analysis can be used to drive the evaluation. For fast validation, we provide the traces collected during our experiment under $data/trace\_*$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected result}

ML-EXray will generate logs in two subfolders: log and nativeLog. log has only high-level performance metrics while nativeLog has per-layer details. Additionally, there is also a summary.log file for per-layer latencies categorized by layer type.

Python scripts under scripts/analysis provides example wrappers to use our Python APIs to parse the logs and reproduce the three major results in the paper: pre-processing bugs, quantization issues, and latency optimization. 

\noindent\textbf{Preprocessing bugs and impact.} To evaluate classification accuracy from EXray logs, please refer to the following

\texttt{\small python3 scripts/analysis/TopKAccuracy.py}

\noindent
We provided example traces (in ./data folder) of the same model running in different configurations (quantized vs. unquantized, BGR input vs RGB input, normalization range of [0,1] vs [-1,1]). The script compares the accuracy of these configurations.

To evaluate your model with different configurations on your own dataset, load your benchmark dataset (e.g. $data/0\_data/imagenet2012\_1$) to your android device under $/sdcard/edgeml/$. Choose your model to run the app. Use adb to pull the logs from the phone. Evaluate the accuracy against your labels.


\noindent\textbf{Debugging quantization issues.} Load your image dataset (follow the format in the image data folder (e.g. data/0\_data/imagenet2012\_1)) into you android device under $/sdcard/edgeml/$. On the app, choose the data source as local and the pasted image folder. Run any model in both quantized and floating point version. Run analysis script comparing the logs.

The following scripts reproduce the result of Mobilenet v2 and v3. Each compares the quantized model's per-layer output against a correct cloud reference pipeline. Note the quantized model can be run using optimized kernels and reference kernels.


\texttt{\scriptsize python3 scripts/analysis/mobilenetv2\_quant\_refop.py}

\texttt{\scriptsize python3 scripts/analysis/mobilenetv3\_quant\_refop.py}


Alternatively, you can also use provided traces and the above scripts to reproduce the results in the paper.

\noindent\textbf{Evaluate per-layer latency.} We build on top of TFLite benchmark tool to evaluate per-layer latency, categorized by layer type. This information is logged in summary.log in each exray trace.

\noindent\textbf{Evaluate system overhead.} Please inspect EXray logs for end-to-end latency with and without logging enabled. To disable logging, specify the argument of EdgeMLMonitor\_Native with no\_logging\_=True.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}
There are two levels of customization: running a new  model on a new hardware to discover unknown behaviors; using ML-EXray APIs to expand logging capability for debugging novel issues.

To run a different model using our demo app, just swap the tflite file in the assets folder and recompile, or use our Python Model Runners to run them on a workstation. Be careful about configurations such as input sizes, pre-processing assumptions, etc. 

ML-EXray is extensible for users to instrument their edge ML pipeline to log custom variables, compare against a custom reference pipeline, and code their own assertion functions.
